A thorough benchmark of automatic text classification: From traditional approaches to large language models

Automatic text classification (ATC) has experienced remarkable advancements in the past decade, best exemplified by recent small and large language models (SLMs and LLMs), leveraged by Transformer architectures. Despite recent effectiveness improvements, a comprehensive cost-benefit analysis investigating whether the effectiveness gains of these recent approaches compensate their much higher costs when compared to more traditional text classification approaches such as SVMs and Logistic Regression is still missing in the literature. In this context, this work's main contributions are twofold: (i) we provide a scientifically sound comparative analysis of the cost-benefit of twelve traditional and recent ATC solutions including five open LLMs, and (ii) a large benchmark comprising {22 datasets}, including sentiment analysis and topic classification, with their (train-validation-test) partitions based on folded cross-validation procedures, along with documentation, and code. The release of code, data, and documentation enables the community to replicate experiments and advance the field in a more scientifically sound manner. Our comparative experimental results indicate that LLMs outperform traditional approaches (up to 26%-7.1% on average) and SLMs (up to 4.9%-1.9% on average) in terms of effectiveness. However, LLMs incur significantly higher computational costs due to fine-tuning, being, on average 590x and 8.5x slower than traditional methods and SLMs, respectively. Results suggests the following recommendations: (1) LLMs for applications that require the best possible effectiveness and can afford the costs; (2) traditional methods such as Logistic Regression and SVM for resource-limited applications or those that cannot afford the cost of tuning large LLMs; and (3) SLMs like Roberta for near-optimal effectiveness-efficiency trade-off.

==> bck/abstractBCK.tex <==
\begin{abstract}



%The field of automatic text classification (ATC) has witnessed an allegedly staggering advance in the last decade due to a profusion of proposals in terms of classification algorithms, most of them motivated or inspired in recent advances regarding the small and large language models (SLMs and LLMs). 
The field of automatic text classification (ATC) has experienced remarkable advancements in the past decade, largely due to numerous proposals for new classification algorithms. Many of these developments have been motivated or inspired by recent breakthroughs in small and large language models (SLMs and LLMs).
%However, this wave of improvements have been shadowed by a cloud of doubts due to a number of potentially (very) problematic issues including (i) use of inadequate experimental protocols; (ii) lack of statistical treatment of the results such as statistical significance tests; (iii) unfair comparison against baselines.
%Therefore, the main contribution of our work is twofold: we provide a comprehensive benchmark comprising 22 datasets and their respective (train-val-test) partitions, enabling the community to compare their approach directly with these results, as well as an up-to-date scientifically sound comparison of traditional and recent ATC solutions. Our \textbf{novelty} relies on the magnitude of the study, the number of experiments and factors analyzed (e.g., datasets, effectiveness, training time), and the employed scientific rigor. 
%second
%Despite the wave of improvements, concerns have arisen due to several potentially problematic issues. These include (i) the use of inadequate experimental protocols, (ii) a lack of statistical analyses of the results, such as tests for statistical significance, and (iii) unfair comparisons against baseline results.
%The main contributions of our work are twofold. %First, we provide a comprehensive benchmark that includes 22 datasets along with their respective train-validation-test partitions. This allows the community to directly compare their approaches with our results. Second, we conduct an up-to-date, scientifically rigorous comparison of both traditional and recent ATC solutions. Our study's novelty lies in its scale, the number of experiments conducted, the variety of factors analyzed (such as datasets, effectiveness, and training time), and the scientific rigor employed throughout the research.
%Despite the wave of improvements, concerns have arisen due to several potentially problematic issues, including a cost-benefit analysis studying if the effectiveness gains of these recent approches in specific tasks compensate the much higher costs related to their applications.
Despite recent improvements, concerns have arisen due to several potentially problematic issues, including a cost-benefit analysis investigating whether the effectiveness gains of these recent approaches in specific tasks compensate the much higher costs associated with their application.
%inadequate experimental protocols, a lack of statistical analyses, and unfair baseline comparisons. 
%the a conclusive cost-benefit analysis of these approaches.
Therefore, our work's main contributions are twofold: we provide an up-to-date scientifically rigorous conclusive analysis of the cost-benefit comparison of \textbf{ten} traditional and recent ATC solutions, as well as a comprehensive benchmark of \textbf{22 datasets} along with their (train-validation-test) partitions, enabling the community for direct comparison.
Our study's novelty lies in its scale, the number of experiments conducted, the variety of factors analyzed (such as datasets, effectiveness, and training time), and the scientific rigor employed throughout the research.
Our experimental results, based on more than \textbf{4000}  measurements, indicate \textbf{TODO}

effectiveness
efficiency.

% reprhase
To ensure reproducibility, our documentation, code, and datasets can be accessed on GitHub -- \url{https://github.com/double-blind}

\end{abstract}

\vspace{-0.3cm}
\keywords{Text Classification, Benchmark, Large Language Models}



V2

\begin{abstract}

The field of automatic text classification (ATC) has experienced remarkable advancements in the past decade, largely due to numerous proposals for new classification algorithms. Many of these developments have been motivated or inspired by recent breakthroughs in small and large language models (SLMs and LLMs).
%Despite recent improvements, concerns have arisen due to several potentially problematic issues, including a cost-benefit analysis investigating whether the effectiveness gains of these recent approaches in specific tasks compensate the much higher costs associated with their application.
Despite recent improvements, a cost-benefit analysis investigating whether the effectiveness gains of these recent approaches in specific tasks compensate the much higher costs associated with their application is still missing in the literature.
Therefore, our work's main contributions are twofold: we provide an up-to-date scientifically rigorous conclusive analysis of the cost-benefit comparison of \textbf{ten} traditional and recent ATC solutions, as well as a comprehensive benchmark of \textbf{22 datasets} along with their (train-validation-test) partitions, enabling the community for direct comparison.
\red{Our experimental results, based on more than \textbf{4000}  measurements, indicate that LLMs outperform traditional approaches (up to XX/on average) and SLMs (up to YY) in classification performance. However, they incur significantly higher computational costs due to fine-tuning, being XXx and YYx slower than traditional methods and SLMs, respectively. 
%The choice between these models remains on the application requirements: best effectiveness (LLMs); cost-efficient (traditional); or a near-optimal tradeoff between effectiveness and efficiency (SLMs).
%We provide a conclusive analysis for choosing among these models based on applications requirements: best effectiveness (LLMs); cost-efficient (traditional); or a near-optimal tradeoff between effectiveness and efficiency (SLMs).
We provide a conclusive analysis based on application needs: best effectiveness (LLMs), cost efficiency (traditional), or near-optimal effectiveness-efficiency trade-off (SLMs).}
%Since LLMs are only X\% more effective on average than SLMs, we conclude that their benefits do not justify the costs.}
To ensure reproducibility, our documentation, code, and datasets can be accessed on GitHub. % -- \url{https://github.com/double-blind}.

\end{abstract}

\vspace{-0.3cm}
\keywords{Text Classification, Benchmark, Large Language Models}


==> bck/atcmethods_bck.tex <==
\textbf{SVM}~\cite{CITE} 
%We adopt the SVM classifier with TFIDF, known for its effectiveness in high-dimensional text representations. For implementation, we use LIBSVM~\cite{chang11}, which supports sequential minimum optimization for optimal Lagrange multipliers. The regularization parameter was selected from eleven values ranging from $2^{-5}$ to $2^{15}$ based on validation sets. TFIDF weights are computed as TF$_i \times$ IDF$_i$, where TF$_i$ is the term frequency, and IDF$_i = \log(\frac{N}{df_i})$, with $N$ being the total document count and $df_i$ the document frequency of term $i$. IDF is calculated using training data only, and the result is normalized using the Euclidean norm (L2 normalization).
is a supervised machine learning algorithm that seeks to find the optimal hyperplane that best separates data into classes. In sum, SVM maximizes the margin between the classes by focusing on the most critical samples, known as support vectors. 
%It can use different kernels (e.g., linear, RBF) to capture complex decision boundaries.

\textbf{LR}~\cite{CITE} is a linear model that predicts the probability of an instance belonging to a particular class using the logistic function. LR learns weights for features to minimize the difference between predicted probabilities and actual labels. %, typically using cross-entropy loss.

\textbf{RF}~\cite{CITE} is an ensemble learning method that builds multiple decision trees during training and aggregates their predictions. % to improve classification accuracy. 
Each tree is trained on a bootstrap sample of the data, and feature splits are chosen randomly, ensuring diversity.

%\textbf{BERT}~\cite{CITE} employs a bidirectional Transformer encoder with 24 blocks, 1024 hidden layers, and 340M parameters. It is pre-trained on a 3.3 billion word corpus, which includes BooksCorpus (800 million words) and English Wikipedia (2.5 billion words). The model predicts missing words in a sentence using two tasks: \textit{Masked language model (MLM)}, where words are masked 15\% of the time, and \textit{Next sentence prediction (NSP)}, which determines if two sentences are consecutive.
\textbf{BERT}~\cite{CITE} employs a bidirectional Transformer encoder with 24 blocks, 1024 hidden layers, and 340M parameters. It was pre-trained on a 3.3 billion word corpus, including BooksCorpus and English Wikipedia. BERT predicts missing words using \textit{Masked language model (MLM)} for 15\% of the words and \textit{Next sentence prediction (NSP)} to assess sentence continuity.

%\textbf{RoBERTa}~\cite{liu2019roberta}  is an end-to-end method that builds on BERT through enhanced fine-tuning with additional data and input manipulations. Key improvements included: i) increased pre-training data; ii) larger mini-batch sizes (up to 32K sequences); iii) extended training time; iv) longer sequence lengths (up to 512); v) modification of the pre-training objective; and vi) dynamic mask generation. RoBERTa was trained on approximately 160GB of English text using 1024 Nvidia 32GB GPUs for about one day, significantly exceeding the original BERT’s computational resources.
\textbf{RoBERTa}~\cite{liu2019roberta} improved BERT by enhancing the fine-tuning with more data and input manipulations. Main improvements include: i) larger pre-training data; ii) mini-batch sizes up to 32K sequences; iii) longer training duration; iv) sequence lengths up to 512; v) changes to the pre-training objective; and vi) dynamic mask generation. %It was trained on about 160GB of English text using 1024 Nvidia 32GB GPUs for roughly one day. %, surpassing the original BERT's resources.

%\textbf{BART}~\cite{lewis2019bart} is a Denoising Autoencoding model that combines features of a bidirectional encoder (like BERT) and an autoregressive decoder (like GPT-2~\cite{CITE}). It introduces noise into the original text using various functions and learns to reconstruct it. The input tokens are replaced with the [MASK] token, and the model's task is to predict these masked tokens. Main noise functions include: i) token masking, ii) token deletion, iii) text infilling, iv) sentence permutation, and v) document rotation.
\textbf{BART}~\cite{lewis2019bart} is a Denoising Autoencoding model that merges a bidirectional encoder (like BERT) with an autoregressive decoder (like GPT~\cite{CITE}). It introduces noise into text and learns to reconstruct it by predicting masked tokens. Key noise functions include: i) token masking, ii) token deletion, iii) text infilling, iv) sentence permutation, and v) document rotation.

\textbf{XLNet}~\cite{yang2019xlnet}: 
%Unlike BERT, which assumes predicted tokens are independent given unmasked tokens, XLNet improves upon this by utilizing a permutation language modeling objective that combines autoregressive and autoencoder benefits. This method was pre-trained on the same parameters and word corpus as BERT, using a massive 32.89B word corpus and trained with 512 TPU v3 chips.
Unlike BERT's independence assumption for predicted tokens, XLNet utilizes a permutation language modeling objective, blending autoregressive and autoencoder advantages. It was pre-trained on the same parameters and corpus as BERT, using a massive 32.89B word corpus and 512 TPU v3 chips.

\textbf{BloomZ}~\cite{CITE} is an extension of the finetuning process for BLOOM and mT5 pretrained multilingual language models applied to a crosslingual task mixture. This family of models has been found capable of crosslingual generalization to unseen tasks and languages.

\textbf{LLaMA}~\cite{CITE} is a family of autoregressive LLMs released by Meta AI. These models are optimized for multilingual dialogue applications and outperform many existing open-source and proprietary chat models on common industry benchmarks. In this work, we focus on two LLaMA versions: LLaMA 2 (7B) and LLaMA 3.1 (8B).





V2


\textbf{SVM}~\cite{CITE} is a supervised machine learning algorithm that seeks to find the optimal hyperplane that best separates data into classes. In sum, SVM maximizes the margin between the classes by focusing on the most critical samples, known as support vectors. 

\textbf{LR}~\cite{CITE} is a linear model that predicts the probability of an instance belonging to a particular class using the logistic function. LR learns weights for features to minimize the difference between predicted probabilities and actual labels. 

\textbf{RF}~\cite{CITE} is an ensemble learning method that builds multiple decision trees during training and aggregates their predictions. Each tree is trained on a bootstrap sample of the data, and feature splits are chosen randomly, ensuring diversity.

\textbf{BERT}~\cite{CITE} employs a bidirectional Transformer encoder with 24 blocks, 1024 hidden layers, and 340M parameters. It was pre-trained on a 3.3 billion word corpus, including BooksCorpus and English Wikipedia. BERT predicts missing words using \textit{Masked language model (MLM)} for 15\% of the words and \textit{Next sentence prediction (NSP)} to assess sentence continuity.

\textbf{RoBERTa}~\cite{liu2019roberta} improved BERT by enhancing the fine-tuning with more data and input manipulations. Main improvements include: i) larger pre-training data; ii) mini-batch sizes up to 32K sequences; iii) longer training duration; iv) sequence lengths up to 512; v) changes to the pre-training objective; and vi) dynamic mask generation.

\textbf{BART}~\cite{lewis2019bart} is a Denoising Autoencoding model that merges a bidirectional encoder (like BERT) with an autoregressive decoder (like GPT~\cite{CITE}). It introduces noise into text and learns to reconstruct it by predicting masked tokens. Key noise functions include: i) token masking, ii) token deletion, iii) text infilling, iv) sentence permutation, and v) document rotation.

\textbf{XLNet}~\cite{yang2019xlnet}: Unlike BERT's independence assumption for predicted tokens, XLNet utilizes a permutation language modeling objective, blending autoregressive and autoencoder advantages. It was pre-trained on the same parameters and corpus as BERT, using a massive 32.89B word corpus and 512 TPU v3 chips.

\textbf{BloomZ}~\cite{CITE} is an extension of the finetuning process for BLOOM and mT5 pretrained multilingual language models applied to a crosslingual task mixture. This family of models has been found capable of crosslingual generalization to unseen tasks and languages.

\textbf{LLaMA}~\cite{CITE} is a family of autoregressive LLMs released by Meta AI. These models are optimized for multilingual dialogue applications and outperform many existing open-source and proprietary chat models on common industry benchmarks. In this work, we focus on two LLaMA versions: LLaMA 2 (7B) and LLaMA 3.1 (8B).




V3=======================




\textbf{SVM}~\cite{CITE} is a supervised machine learning algorithm that seeks to find the optimal hyperplane that best separates data into classes. In sum, SVM maximizes the margin between the classes by focusing on the most critical samples, known as support vectors. 

\textbf{LR}~\cite{CITE} is a linear model that predicts the probability of an instance belonging to a particular class using the logistic function. LR learns weights for features to minimize the difference between predicted probabilities and actual labels. 

\textbf{RF}~\cite{CITE} is an ensemble learning method that builds multiple decision trees during training and aggregates their predictions. Each tree is trained on a bootstrap sample of the data, and feature splits are chosen randomly, ensuring diversity.

\textbf{BERT}~\cite{CITE} employs a bidirectional Transformer encoder with 24 blocks, 1024 hidden layers, and 340M parameters. %It was pre-trained on a 3.3 billion word corpus, including BooksCorpus and English Wikipedia. 
BERT predicts missing words using \textit{Masked language model (MLM)} for 15\% of the words and \textit{Next sentence prediction (NSP)} to assess sentence continuity.

\textbf{RoBERTa}~\cite{liu2019roberta} improved BERT by enhancing the fine-tuning with more data and input manipulations. Main improvements include: i) larger pre-training data; ii) mini-batch sizes up to 32K sequences; iii) longer training duration; iv) sequence lengths up to 512; v) changes to the pre-training objective; and vi) dynamic mask generation.

\textbf{BART}~\cite{lewis2019bart} is a Denoising Autoencoding model that merges a bidirectional encoder (like BERT) with an autoregressive decoder (like GPT~\cite{CITE}). It introduces noise into text and learns to reconstruct it by predicting masked tokens. Key noise functions include: i) token masking, ii) token deletion, iii) text infilling, iv) sentence permutation, and v) document rotation.

\textbf{XLNet}~\cite{yang2019xlnet}: Unlike BERT's independence assumption for predicted tokens, XLNet utilizes a permutation language modeling objective, blending autoregressive and autoencoder advantages. It was pre-trained on the same parameters and corpus as BERT, using a massive 32.89B word corpus and 512 TPU v3 chips.

\textbf{BloomZ}~\cite{CITE} is an extension of the finetuning process for BLOOM and mT5 pretrained multilingual language models applied to a crosslingual task mixture. This family of models has been found capable of crosslingual generalization to unseen tasks and languages.

\textbf{LLaMA}~\cite{CITE} is a family of autoregressive LLMs released by Meta AI. These models are optimized for multilingual dialogue applications and outperform many existing open-source and proprietary chat models on common industry benchmarks. In this work, we focus on two LLaMA versions: LLaMA 2 (7B) and LLaMA 3.1 (8B).





V4 +===================================


\textbf{SVM}~\cite{CITE} is a supervised machine learning algorithm that seeks to find the optimal hyperplane that best separates data into classes. In sum, SVM maximizes the margin between the classes by focusing on the most critical samples, known as support vectors. 

\textbf{LR}~\cite{CITE} is a linear model that predicts the probability of an instance belonging to a particular class using the logistic function. LR learns weights for features to minimize the difference between predicted probabilities and actual labels. 

\textbf{RF}~\cite{CITE} is an ensemble learning method that builds multiple decision trees during training and aggregates their predictions. Each tree is trained on a bootstrap sample of the data, and feature splits are chosen randomly, ensuring diversity.

\textbf{BERT}~\cite{CITE} employs a bidirectional Transformer encoder with 24 blocks, 1024 hidden layers, and 340M parameters. %It was pre-trained on a 3.3 billion word corpus, including BooksCorpus and English Wikipedia. 
BERT predicts missing words using \textit{Masked language model} for 15\% of the words and \textit{Next sentence prediction} to assess sentence continuity.

\textbf{RoBERTa}~\cite{liu2019roberta} improved BERT by enhancing the tuning with more data and input manipulations, including: i) larger pre-training data; ii) mini-batch sizes up to 32K sequences; iii) longer training duration; iv) sequence lengths up to 512; v) changes to the pre-training objective; and vi) dynamic mask generation.

\textbf{BART}~\cite{lewis2019bart} is a Denoising Autoencoding model that merges a bidirectional encoder with an autoregressive decoder. It introduces noise into text and learns to rebuild it by predicting masked tokens. %Key noise functions include: i) token masking, ii) token deletion, iii) text infilling, iv) sentence permutation, and v) document rotation.
\looseness=-1

\textbf{XLNet}~\cite{yang2019xlnet}: Unlike BERT's independence assumption for predicted tokens, XLNet utilizes a permutation language modeling objective, blending autoregressive and autoencoder advantages. %It was pre-trained on the same parameters and corpus as BERT, using a massive 32.89B word corpus and 512 TPU v3 chips.

\textbf{BloomZ}~\cite{CITE} is an extension of the finetuning process for BLOOM and mT5 pretrained multilingual language models applied to a crosslingual task mixture. This family of models has been found capable of crosslingual generalization to unseen tasks and languages.

\textbf{LLaMA}~\cite{CITE} is a family of autoregressive LLMs released by Meta AI. These models are optimized for multilingual dialogue applications and outperform many existing open-source and proprietary chat models on common industry benchmarks. In this work, we focus on two LLaMA versions: LLaMA 2 (7B) and LLaMA 3.1 (8B).






V5 +=================================



**SVM**~\cite{CITE} is a supervised learning algorithm that identifies the optimal hyperplane for separating classes by maximizing the margin from critical samples, known as support vectors.

**LR**~\cite{CITE} is a linear model that predicts the probability of class membership using the logistic function, adjusting feature weights to minimize the error between predicted probabilities and actual labels.

**RF**~\cite{CITE} is an ensemble method that constructs multiple decision trees during training, using bootstrap samples and random feature splits to ensure diversity in predictions.

**BERT**~\cite{CITE} utilizes a bidirectional Transformer encoder to predict missing words via a masked language model and assess continuity through next sentence prediction.

**RoBERTa**~\cite{liu2019roberta} enhances BERT by using larger pre-training data, longer training durations, and dynamic mask generation to improve performance.

**BART**~\cite{lewis2019bart} is a Denoising Autoencoder that combines a bidirectional encoder with an autoregressive decoder to reconstruct text from input noise.

**XLNet**~\cite{yang2019xlnet} employs a permutation language modeling objective, integrating autoregressive and autoencoder benefits to predict tokens without independence assumptions.

**BloomZ**~\cite{CITE} extends the finetuning of BLOOM and mT5 multilingual models, enabling crosslingual generalization across unseen tasks and languages.

**LLaMA**~\cite{CITE} is a family of autoregressive language models by Meta AI, optimized for multilingual dialogue and surpassing many benchmarks. This work focuses on LLaMA 2 (7B) and LLaMA 3.1 (8B).


==> resource/tables/datasets_stats.tex <==
%\begin{table*}[!ht]
\begin{table*}[h]
    \centering
    \scriptsize
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{llrrrrrrrrrrrrr}
        \toprule
 %                     &           &             & \multicolumn{5}{c}{ Class Distribution }                                                                                                \\ \vspace{0.005cm}
 %       \cline{4-10}
        %Task & Dataset       & Size      & Dimensionality & \# Classes  &  \begin{tabular}{@{}c@{}}Avg Doc. \\ Length (words) \end{tabular} \\ % & Skewness              \\
        &  &           &             & \multicolumn{5}{c}{ Class Distribution }                                                                                                \\
        \cline{5-9} 
        Task & Dataset       & Size      & Dim. & \# Classes  &  Minor & Median    & Mean      & Major & Density  & Skewness    \\
        \midrule
  \parbox[t]{1mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{Topic}}} & DBLP & 38,128 & 28,131 & 10 & 1,414 & 3,590 & 3,812 & 9,746 & 141 & Imbalanced \\
 & Books & 33,594 & 46,382 & 8 & 1,226 & 4,534 & 4,199 & 4,934 & 269 & Imbalanced \\
 & ACM & 24,897 & 48,867 & 11 & 63 & 2,041 & 2,263 & 6,562 & 65 & Imbalanced   \\
 & 20NG & 18,846 & 97,401 & 20 & 628 & 984 & 942 & 999 & 96 & Balanced    \\
 & OHSUMED & 18,302 & 31,951 & 23 & 56 & 592 & 795 & 2,876 & 154 & Imbalanced   \\
 & Reuters90 & 13,327 & 27,302 & 90 & 2 & 29 & 148 & 3,964 & 171 & Extremely   Imbalanced \\
 & WOS-11967 & 11,967 & 25,567 & 33 & 262 & 371 & 362 & 449 & 195 & Balanced \\
 & WebKB & 8,199 & 23,047 & 7 & 137 & 926 & 1,171 & 3,705 & 209 & Imbalanced   \\
 & TREC & 5,952 & 3,032 & 6 & 95 & 1,148 & 992 & 1,344 & 10 & Imbalanced \\ 
 & WOS-5736 & 5,736 & 18,031 & 11 & 380 & 426 & 521 & 750 & 201 & Balanced \\ \hline
\parbox[t]{1mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Sentiment}}} & SST1 & 11,855 & 9,015 & 5 & 1,510 & 2,242 & 2,371 & 3,140 & 19 & Balanced         \\
 & pang\_movie & 10,662 & 17,290 & 2 & 5,331 & 5,331 & 5,331 & 5,331 & 21 & Balanced        \\
 & Movie Review & 10,662 & 9,070 & 2 & 5,331 & 5,331 & 5,331 & 5,331 & 21 & Balanced   \\
 & vader\_movie & 10,568 & 16,827 & 2 & 5,242 & 5,284 & 5,284 & 5,326 & 19 & Balanced        \\
 & MPQA & 10,606 & 2,643 & 2 & 3,312 & 5,303 & 5,303 & 7,294 & 3 & Imbalanced         \\
 & Subj & 10,000 & 10,151 & 2 & 5,000 & 5,000 & 5,000 & 5,000 & 24 & Balanced         \\
 & SST2 & 9,613 & 7,866 & 2 & 4,650 & 4,806 & 4,806 & 4,963 & 19 & Balanced         \\
 & yelp\_reviews & 5,000 & 23,631 & 2 & 2,500 & 2,500 & 2,500 & 2,500 & 132 & Balanced        \\
 & vader\_nyt & 4,946 & 12,004 & 2 & 2,204 & 2,473 & 2,473 & 2,742 & 18 & Balanced        \\
  %Cade12 & 40,983 & 80,897 & 13                              &   &   &   &   & 116                                    &   Imbalanced \\
  %vader\_twitter         &  4,196    &    8,344     &   2    &   &   &   &   &   14      &   Balanced        \\
  %vader\_amazon          &  3,610    &    4,687     &   2    &   &   &   &   &   17      &   Balanced        \\
  %tweet\_semevaltest     &  3,060    &    9,548     &   2    &   &   &   &   &   20      &   Balanced        \\
  %sentistrength\_twitter &  2,289    &    8,023     &   2    &   &   &   &   &   16      &   Balanced        \\
  %sentistrength\_youtube &  2,432    &    6,867     &   2    &   &   &   &   &   17      &   Balanced        \\


        \bottomrule
    \end{tabular}
    }
    \caption{Datasets Statistics}
    \label{tbl:datasets_stats}
\end{table*}
